RefGC-SR$^2$: Reference-guided Super-Resolution and Refinement of AI Generated Content

Reference-guided generation (e.g., object compositing, customization) has progressed rapidly, yet current pipelines share a fundamental limitation: the object-centric high-resolution reference image (HRRI) provided by users is downsampled to a fixed low-resolution (LR) before being fed into the model, so the fine-grained details are discarded before the output is even produced. In addition, the generation step then introduces its own artifacts (e.g., identity distortion) on top of this loss. Existing reference-guided generated content refinement (RefGCR) methods can correct some of these artifacts but still operate in the LR domain; reference-guided super-resolution (RefSR) methods recover resolution but assume natural-image degradations and ignore the artifact distribution of generative pipelines. To address both gaps in a single formulation, we introduce a new task: reference-guided generated content super-resolution-refinement (RefGC-SR$^2$), where the original HRRI is reused at the post-processing stage to recover lost details, refine generative artifacts, and upscale the output simultaneously. We construct the first real-world triplet data generation pipeline for this RefGC-SR$^2$ task, training a diptych-conditioned generator to synthesize paired low-quality anchors that public pretrained models cannot provide. We further present a frequency-aware diffusion transformer model for RefGC-SR$^2$ that selectively injects fine details from the HRRI while removing generative artifacts. Extensive experiments demonstrate that our RefGC-SR$^2$ model successfully (i) refines the object identity faithfully with respect to the reference, and (ii) recovers high-resolution details, so that the final result is significantly higher quality and practically more usable compared to existing RefGCR and RefSR baselines.

==> cmlab_preamble.tex <==
% =================================================================
% CMLab arXiv Paper Template - Preamble (cmlab-specific only)
% =================================================================
% This file contains only the packages and settings required for
% applying the cmlab paper template. General academic packages
% (graphicx, algorithm, etc.) needed for writing your own paper
% should be added directly in main.tex after \input{cmlab_preamble}.
%
% Contents of this file:
%   1. XeLaTeX compatibility shim (handles pdfTeX-only packages
%      like axessibility)
%   2. cmlab theme colors (#0D207F navy)
%   3. hyperref setup (link colors)
%   4. cleveref two-color system (Sec.(dark) 3.2(light))
%   5. cmlab_1.sty invocation (cover-box design)
% =================================================================


% -----------------------------------------------------------------
% 1. XeLaTeX/LuaLaTeX compatibility shim
% -----------------------------------------------------------------
% Define pdfTeX-only commands as no-ops so packages like axessibility
% (which rely on pdfTeX internals) still compile under XeLaTeX.
% Under pdfLaTeX this block does nothing.
\RequirePackage{iftex}
\ifPDFTeX\else
  \newcount\pdfcompresslevel
  \newcount\pdfoptionpdfminorversion
  \newcount\pdfgentounicode
  \providecommand{\pdfcatalog}[1]{}
  \providecommand{\pdfglyphtounicode}[2]{}
\fi


% -----------------------------------------------------------------
% 2. cmlab theme colors
% -----------------------------------------------------------------
%   cmlabPrefix : Color for prefixes (Sec. / Fig. / Tab. / Eq.) — dark navy
%   cmlabNumber : Color for numbers (1, 3.2, (5))                — light navy
%   cmlabCite   : Color for \cite
%   cmlabURL    : Color for \url, \href
\usepackage{xcolor}
\definecolor{cmlabPrefix}{HTML}{0D207F}  % cmlab dark navy
% \definecolor{cmlabNumber}{HTML}{7386E6}  % cmlab light navy (alternative)
\definecolor{cmlabNumber}{HTML}{0D207F}  % cmlab dark navy (unified single color)
\definecolor{cmlabCite}{HTML}{0D207F}    % cite also dark navy
\definecolor{cmlabURL}{HTML}{0D207F}     % URL also dark navy


% -----------------------------------------------------------------
% 3. hyperref setup (link colors)
% -----------------------------------------------------------------
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,
  linkcolor=cmlabNumber,    % Number color for \ref (cref is redefined below)
  citecolor=cmlabCite,      % \cite (references)
  urlcolor=cmlabURL,        % \url, \href (external URLs)
  filecolor=cmlabURL,
  pdfborder={0 0 0},
}


% -----------------------------------------------------------------
% 4. cleveref: unified reference output ("Fig. 5", "Table 1") via \cref{...}
% -----------------------------------------------------------------
% Must be loaded AFTER hyperref.
\usepackage[capitalize,noabbrev]{cleveref}


% -----------------------------------------------------------------
% 5. cleveref format override — separate colors for prefix and number
% -----------------------------------------------------------------
% Style:
%   "Sec. 3.2"  ->  Sec.(dark navy) + 3.2(light navy)
%
% cleveref \crefformat arguments:
%   #1 : Reference number (e.g., 3.2, 1, (5))
%   #2 : hyperref link begin
%   #3 : hyperref link end
%
% Helper macro \cmlabRef{prefix}{#1}{#2}{#3}
%   - prefix part: cmlabPrefix color
%   - number part: cmlabNumber color
%   - hyperref clickable area preserved
\newcommand{\cmlabRef}[4]{%
  {\color{cmlabPrefix}#1}~#3{\color{cmlabNumber}#2}#4%
}
\newcommand{\cmlabRefParen}[4]{% For equations: wrap number in (...)
  {\color{cmlabPrefix}#1}~#3{\color{cmlabNumber}(#2)}#4%
}

% --- figure ---
\crefformat{figure}     {\cmlabRef{Fig.}{#1}{#2}{#3}}
\Crefformat{figure}     {\cmlabRef{Figure}{#1}{#2}{#3}}
\crefrangeformat{figure}%
  {{\color{cmlabPrefix}Figs.}~#3{\color{cmlabNumber}#1}#4--#5{\color{cmlabNumber}#2}#6}
\crefmultiformat{figure}%
  {\cmlabRef{Figs.}{#1}{#2}{#3}}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, and #2{\color{cmlabNumber}#1}#3}

% --- table ---
\crefformat{table}      {\cmlabRef{Tab.}{#1}{#2}{#3}}
\Crefformat{table}      {\cmlabRef{Table}{#1}{#2}{#3}}
\crefrangeformat{table}%
  {{\color{cmlabPrefix}Tabs.}~#3{\color{cmlabNumber}#1}#4--#5{\color{cmlabNumber}#2}#6}
\crefmultiformat{table}%
  {\cmlabRef{Tabs.}{#1}{#2}{#3}}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, and #2{\color{cmlabNumber}#1}#3}

% --- section / subsection / subsubsection ---
\crefformat{section}    {\cmlabRef{Sec.}{#1}{#2}{#3}}
\Crefformat{section}    {\cmlabRef{Section}{#1}{#2}{#3}}
\crefformat{subsection} {\cmlabRef{Sec.}{#1}{#2}{#3}}
\Crefformat{subsection} {\cmlabRef{Section}{#1}{#2}{#3}}
\crefformat{subsubsection}{\cmlabRef{Sec.}{#1}{#2}{#3}}
\Crefformat{subsubsection}{\cmlabRef{Section}{#1}{#2}{#3}}
\crefrangeformat{section}%
  {{\color{cmlabPrefix}Secs.}~#3{\color{cmlabNumber}#1}#4--#5{\color{cmlabNumber}#2}#6}
\crefmultiformat{section}%
  {\cmlabRef{Secs.}{#1}{#2}{#3}}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, and #2{\color{cmlabNumber}#1}#3}

% --- equation ---
\crefformat{equation}   {\cmlabRefParen{Eq.}{#1}{#2}{#3}}
\Crefformat{equation}   {\cmlabRefParen{Equation}{#1}{#2}{#3}}
\crefrangeformat{equation}%
  {{\color{cmlabPrefix}Eqs.}~#3{\color{cmlabNumber}(#1)}#4--#5{\color{cmlabNumber}(#2)}#6}
\crefmultiformat{equation}%
  {\cmlabRefParen{Eqs.}{#1}{#2}{#3}}%
  {, #2{\color{cmlabNumber}(#1)}#3}%
  {, #2{\color{cmlabNumber}(#1)}#3}%
  {, and #2{\color{cmlabNumber}(#1)}#3}

% --- algorithm ---
% Unlike amsmath, \usepackage{algorithm} uses 'algorithm' as the counter name.
% (If the algorithm package is not used, this block is harmless.)
\crefname{algorithm}{Algo.}{Algos.}
\Crefname{algorithm}{Algorithm}{Algorithms}
\crefformat{algorithm}  {\cmlabRef{Algo.}{#1}{#2}{#3}}
\Crefformat{algorithm}  {\cmlabRef{Algorithm}{#1}{#2}{#3}}
\crefrangeformat{algorithm}%
  {{\color{cmlabPrefix}Algos.}~#3{\color{cmlabNumber}#1}#4--#5{\color{cmlabNumber}#2}#6}
\crefmultiformat{algorithm}%
  {\cmlabRef{Algos.}{#1}{#2}{#3}}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, and #2{\color{cmlabNumber}#1}#3}

% \cite is colored automatically via hyperref's citecolor=cmlabCite.
% No additional hook needed (same approach as the SANA-WM paper).


% -----------------------------------------------------------------
% 6. CMLab public/arXiv title-box style
% -----------------------------------------------------------------
% arXiv public version : turn on the 'enable' option → use cmlab cover box
% Conference camera-ready : remove 'enable' → use the venue's \maketitle
\usepackage[
  enable,
  applybold,                              % Apply Ubuntu font to all bold text (section headings, caption labels, \textbf, ...)
  labname={CMLab},
  leftlogo={./assets/adobe.png},      % Bottom-left logo (affiliation / collaborator)
  logo={./assets/cmlab_logo.png},         % Bottom-right logo (CMLab)
  titleicon={./assets/icon.png},          % Icon shown next to the title (optional)
  logowidth={21mm},
  projectpage={https://cmlab-korea.github.io/CHIMERA/}
]{cmlab_1}

% For the camera-ready version, replace the \usepackage[...]{cmlab_1} block
% above with the following (drop the 'enable' option):
% \usepackage[
%   labname={CMLab},
%   logo={assets/cmlab_logo.png},
%   titleicon={assets/icon.png},
%   logowidth={22mm},
%   projectpage={https://cmlab-korea.github.io/CHIMERA/}
% ]{cmlab_1}

